Measuring Forecasting Skill from Text

People vary in their ability to make accurate predictions about the future. Prior studies have shown that some individuals can predict the outcome of future events with consistently better accuracy. This leads to a natural question: what makes some forecasters better than others? In this paper we explore connections between the language people use to describe their predictions and their forecasting skill. Datasets from two different forecasting domains are explored: (1) geopolitical forecasts from Good Judgment Open, an online prediction forum and (2) a corpus of company earnings forecasts made by financial analysts. We present a number of linguistic metrics which are computed over text associated with people's predictions about the future including: uncertainty, readability, and emotion. By studying linguistic factors associated with predictions, we are able to shed some light on the approach taken by skilled forecasters. Furthermore, we demonstrate that it is possible to accurately predict forecasting skill using a model that is based solely on language. This could potentially be useful for identifying accurate predictions or potentially skilled forecasters earlier.

==> related.tex <==
%!TEX root = main.tex

\section{Related Work}

Many recent studies have analyzed connections between users' language and human attributes \cite{hovy2015user,nguyen2013old,volkova2014inferring, Tan:2016:WAI:2872427.2883081, ICWSM148106}.
\citet{son2018causal} developed a tool for discourse analysis in social media and found that older individuals and females tend to use more causal explanations.
Another example is work by \citet{schwartz2015extracting}, who developed automatic classifiers for temporal orientation and found important differences relating to age, gender in addition to Big Five personality traits.
\citet{eichstaedt2015psychological} showed that language expressed on Twitter can be predictive of community-level psychological correlates, in addition to rates of heart disease.
\citet{graham-liu-2016-achieving} analyzed political polarization in social media and \citet{voigt2017language} examined the connections between police officers' politeness and race by analyzing language.
A number of studies \cite{DeChoudhury:2014:CPP:2531602.2531675,Eichstaedt11203,benton2017multitask,park2017living} have examined the connection between users' language on social media and depression and alcohol use \cite{using-longitudinal}. 
Other work has analyzed users' language to study the effect of attributes, such as gender, in online communication \citep{bamman2014gender,wang-jurgens-2018-going,voigt2018rtgender}.  In this work we study the relationship between people's language and their forecasting skill. To the best of our knowledge, this is the first work that presents a computational way of exploring this direction.

Our work is also closely related to prior research on predicting various phenomenon from users' language.  For example \citet{tan-etal-2014-effect} study the effect of wording on message propagation, \citet{gillick2018please} examine the connection between language used by politicians in campaign speeches and applause and \citet{perez2015experiments} explored linguistic differences between truthful and deceptive statements.  \citet{ganjigunte-ashok-etal-2013-success} show linguistic cues drawn from authors' language are strong indicators of the success of their books and \citet{tsur2009revrank} presented an unsupervised model to analyze the helpfulness of book reviews by analyzing their text.

There have been several studies using data from Good Judgment Open or Good Judgment Project \cite{mellers2015identifying}. 
One recent study examining the language side of this data is \citet{schwartz-etal-2017-assessing}.
Their main goal is to suggest objective metrics as alternatives for subjective ratings when evaluating the quality of recommendations. %(e.g., restaurant reviews).
% , as subjective ratings are often biased. 
To achieve this, justifications written by one group are provided as tips to another group.  These justifications are then evaluated on their ability to persuade people to update their predictions, leading to \textit{real} benefits that can be measured by objective metrics. Prior work has also studied persuasive language on crowdfunding platforms \citep{yang2019let}.
% (better forecasting accuracy in their setting).
In contrast, our work focuses on directly measuring forecasting skill based on text justifications. 
% It is clear that justifications having actual benefits do not necessarily need to come from accurate forecasts or good forecasters.

Finally we note that there is a long history of research on financial analysts' forecasting ability \citep{10.2307/245673, 10.2307/4480122, LOH2006455}. Most work relies on regression models to test if pre-identified factors are correlated with forecasting skill (e.g., \citet{LOH2006455, Call2009}). Some work has also explored the use of textual information in financial domain.  For example, \citet{kogan-etal-2009-predicting} present a study of predicting companies' risk by using financial reports. We also note a recent paper on studying financial analysts' decision making process by using text-based features from earning calls \cite{keith-stent-2019-modeling}. As far as we aware, our work is the first to evaluate analysts' forecasting skill based on their language.
